Enhanced Signal Recovery via Sparsity Inducing Image Priors

Parsimony in signal representation is a topic of active research. Sparse signal processing and representation is the outcome of this line of research which has many applications in information processing and has shown significant improvement in real-world applications such as recovery, classification, clustering, super resolution, etc. This vast influence of sparse signal processing in real-world problems raises a significant need in developing novel sparse signal representation algorithms to obtain more robust systems. In such algorithms, a few open challenges remain in (a) efficiently posing sparsity on signals that can capture the structure of underlying signal and (b) the design of tractable algorithms that can recover signals under aforementioned sparse models.

==> Chapter-RoadMap/Chapter-RoadMap.tex <==
\chapter{Roadmap}
\label{chapter:roadmap}

\begin{itemize}
\item Ph.D. candidacy exam: Jan 2013
\item Ph.D. comprehensive exam: May 2015
\item Contribution I towards thesis
\begin{itemize}
\item Conference paper published and presented; journal draft under preparation
\end{itemize}
\item Contribution II towards thesis
\begin{itemize}
\item Journal paper under review
\end{itemize}
\item Contribution III towards thesis
\begin{itemize}
\item Formulation of ideas, conference paper under preparation
\end{itemize}
\item Expected date of graduation: May 2017.
\end{itemize}


==> Miscellaneous/doc16.tex <==
@string{
    ap_acha = "Applied and Computational Harmonic Analysis"
}

@string{
    ieee_tcas2 = "IEEE Trans. on Circuits and Systems---II: Analog and Digital Signal Processing"
}

@string{
    ieee_tsp = "IEEE Trans. on Signal Processing"
}

@string{
    ieee_tip = "IEEE Trans. on Image Processing"
}

@string{
    ieee_tit = "IEEE Trans. on Information Theory"
}

@string{
    ieee_tcas = "IEEE Trans. on Circuits and Systems"
}

@string{
    ieee_tpami = "IEEE Trans. on Pattern Analysis and Machine Intelligence"
}

@string{
    ieee_tassp = "IEEE Trans. on Acoustics, Speech, and Signal Processing"
}

@string{
    ieee_tgrs = "IEEE Trans. on Geoscience and Remote Sensing"
}

@string{
    ieee_pacrim = "Proc. of IEEE Pacific Rim Conference on Communications,
      Computers and Signal Processing"
}

@string{
    ieee_icip = "Proc. of IEEE International Conference on Image Processing"
}


@string{
    ieee_icassp = "Proc. of IEEE Int. Conf. Acoust., Speech, Signal Process."
}

@string{
    ieee_cvpr = "Proc. of IEEE Conf. Comput. Vision Pattern Recognition"
}

@string{
    ieee_iscas = "Proc. of IEEE Int. Symp. Circuits and Systems"
}

@string{
    spie_vcip = "Proc. of SPIE Visual Commun. Image Process."
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Publications
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{
    Wright_2009,
    author = "J. Wright and A. Y. Yang and A. Ganesh and S. Sastry and Y. Ma",
    title = "Robust Face Recognition via Sparse Representation",
    journal = IEEE_J_PAMI,
    volume = 31,
    number = 2,
    month = feb,
    year = 2009,
    pages = "210--227"
}

@article{
    Hang_2009,
    author = "X. Hang and F.-X. Wu",
    title = "Sparse Representation for Classification of Tumors Using Gene Expression Data",
    journal = "Journal of Biomedicine and Biotechnology",
    volume = 2009,
    year = 2009,
    note = "doi:10.1155/2009/403689"
}

@inproceedings{
    Pillai_2009,
    author = "J. K. Pillai and V. M. Patel and R. Chellappa",
    title = "Sparsity Inspired selection and recognition of iris images",
    booktitle = "Proc. IEEE Third Int. Conf. Biometrics: Theory, Applications and Systems",
    year = 2009,
    month = sep,
    address = "Washington D.C.",
    pages = "1--6"
}

@article{
    Pillai_2011,
    author = "J. K. Pillai and V. M. Patel and R. Chellappa and N. Ratha",
    title = "Secure and robust iris recognition using Sparse Representations and Random Projections",
    journal = IEEE_J_PAMI,
    volume = 33,
    number = 9,
    month = sep,
    year = 2011,
    pages = "1877--1893"
}


@inproceedings{
    Do_2009,
    author = "T. T. Do and Y. Chen and D. T. Nguyen and N. H. Nguyen and L. Gan and T. D. Tran",
    title = "Distributed compressed video sensing",
    booktitle = "Proc. {IEEE} Int. Conf. Image Process.",
    month = nov,
    year = 2009,
    pages = "1393-1396",
    address = "Cairo, Egypt"
}


@article{
    Basri_2003,
    author = "R. Basri and D. W. Jacobs",
    title = "Lambertian Reflectance and Linear Subspaces",
    journal = IEEE_J_PAMI,
    volume = 25,
    number = 2,
    month = feb,
    year = 2003,
    pages = "218-233"
}

@Article{
    CandesRob06,
    author = "E. Cand\`{e}s and J. Romberg and T. Tao",
    title =  "Robust uncertainty principles: Exact signal reconstruction from highly incomplete frequency information",
    journal = IEEE_J_IT,
    volume =  52,
    number = 2,
    month = Feb,
    year = 2006,
    pages = "489-509"
}

@Article{
    Zhao_2003,
    author = "W. Zhao and R. Chellappa and P.~J. Phillips and A. Rosenfeld",
    title =  "Face Recognition: A Literature Survey",
    journal = "ACM Computing Surveys",
    volume =  35,
    number = 4,
    month = dec,
    year = 2003,
    pages = "399-458"
}

@inproceedings{
    Wagner_2009,
    author = "A. Wagner and J. Wright and A. Ganesh and Z. Zhou and Y. Ma",
    title = "Towards a practical face recognition system: Robust registration and illumination by sparse representation",
    booktitle = ieee_cvpr,
    pages = "597-604",
    month = jun,
    year = 2009,
    address = "Miami, FL"
}

@inproceedings{
    Huang_2008,
    author = "J. Huang and X. Huang and D. Metaxas",
    title = "Simultaneous image transformation and sparse representation recovery",
    booktitle = ieee_cvpr,
    pages = "1-8",
    month = jun,
    year = 2008,
    address = "Anchorage, AK"
}

@article{Tropp_2005,
  author = "J. Tropp and A. Gilbert",
  title =  "Signal recovery from random measurements via Orthogonal Matching Pursuit",
  journal = IEEE_J_IT,
  volume =   53,
  number = 12,
  month =    dec,
  year =     2007,
  pages =    "4655-4666"
}

@article{Dai_2009,
  author = "W. Dai and O. Milenkovic",
  title =  "Subspace Pursuit for Compressive Sensing Signal Reconstruction",
  journal = IEEE_J_IT,
    volume = 55,
    number = 5,
    month = may,
    year = 2009,
    pages = "2230-2249"
}

@inproceedings{
    Guo_2009,
    author = "Z. Guo and T. Wittman and S. Osher",
    title = "L1 unmixing and its application to hyperspectral image enhancement",
    booktitle = "Proc. SPIE Conf. on Algorithms and Technologies for Multispectral, Hyperspectral, and Ultraspectral Imagery XV.",
    volume = 7334,
    month = apr,
    year = 2009,
    address = "Orlando, FL"
}

@article{GeBeKr01,
  author =  "A. S. Georghiades and P. N. Belhumeur and D. J. Kriegman",
  title =   "From Few to Many: Illumination Cone Models for Face Recognition under Variable Lighting and Pose",
  journal = IEEE_J_PAMI,
  month = jun,
  year =  2001,
  volume = 23,
  number = 6,
  pages= "643-660"
  }

@article{Aharon_2006,
  author =  "M. Aharon and M. Elad and A. M. Bruckstein",
  title =   "K-SVD: An algorithm for designing overcomplete dictionaries for sparse representation",
  journal = IEEE_J_SP,
  month = nov,
  year =  2006,
  volume = 54,
  number = 11,
  pages= "4311-4322"
  }

@article{Elad_2006,
  author =  "M. Elad and M. Aharon",
  title =   "Image denoising via sparse and redundant representations over learned dictionaries",
  journal = IEEE_J_IP,
  month = dec,
  year =  2006,
  volume = 15,
  number = 12,
  pages= "3736-3745"
  }

@article{ARDatabase,
  author =  "A.~M. Martinez and R. Benavente",
  title =   {{The AR face database}},
  journal = "CVC Tech. Report",
  year =  1998,
  number = 24
  }

@article{Sirovich_1987,
  author =  "L. Sirovich and M. Kirby",
  title =   "Low-dimensional procedure for the characterization of human faces",
  journal = {J. Optical Soc. of Am. A},
  month = mar,
  year =  1987,
  volume = 4,
  number = 3,
  pages= "519-524"
  }

@article{Turk_1991,
    author = "M. Turk and A. Pentland",
    title = "Eigenfaces for recognition",
    journal = {J. Cogn. Neurosci.},
    volume = 3,
    number = 1,
    month = {Winter},
    year = 1991,
    pages = "71-86"
}

@PHDTHESIS{Shashua_1992,
    AUTHOR = "A. Shashua",
    TITLE = {{Geometry and photometry in 3D visual recognition}},
    SCHOOL = "MIT",
    YEAR ="1992"}

@article{Belhumeur_1997,
    author = "P.~N. Belhumeur and J.~P. Hespanha and D.~J. Kriegman",
    title = "Eigenfaces vs. Fisherfaces: Recognition using class specific linear projection",
    journal = IEEE_J_PAMI,
    volume = 19,
    number = 7,
    month = jul,
    year = 1997,
    pages = "711-720"
}

@article{Kittler98,
  author    =   {J. Kittler and M. Hatef and R.~P.~W. Duin and J. Matas},
  title     =   {On combining classifiers},
  journal   =   IEEE_J_PAMI,
  year      =   {1998},
  month     =   mar,
  volume    =   {20},
  number    =   {3},
  pages     =   {226-239}
}

@inproceedings{discGM:Srinivas11,
  author    = "Umamahesh Srinivas and Vishal Monga and Raghu G.~Raj",
  title     = "Automatic target recognition using discriminative graphical models",
  booktitle = "Proc. {IEEE} Intl. Conf. Image Processing",
  pages     = {33-36},
  month = sep,
  year      = 2011,
  address = "Brussels, Belgium"
}

@inproceedings{Chen_2009,
    author = "Y. Chen and T.~T. Do and T.~D. Tran",
    title = "Robust face recognition using locally adaptive sparse representation",
    booktitle = "Proc. {IEEE} Intl. Conf. Image Processing",
    year = 2011,
    pages = {1657-1660},
    month = sep,
    address = "Hong Kong"
}

@inproceedings{Do_2008,
    author = "T. T. Do and L. Gan and N. H. Nguyen and T. D. Tran",
    title = "Sparsity adaptive matching pursuit algorithm for practical compressed sensing",
    booktitle = "Proc. IEEE Asilomar Conf. on Signals, Systems, and Computers",
    month = oct,
    year = 2008,
    pages = "581-587",
    address = "Pacific Grove, CA"
}

@article{Tan10,
  author    =   {V.~Y.~F. Tan and S. Sanghavi and J.~W. Fisher III and A.~S. Willsky},
  title     =   {Learning graphical models for hypothesis testing and classification},
  journal   =   "IEEE Trans. Signal Processing",
  month     = 	nov,
  year      =   2010,
  volume    =   58,
  number    =   11,
  pages     =   "5481-5495"
}

@book{Lauritzen96,
  title     =   {{Graphical Models}},
  publisher =   {Oxford University Press, NY},
  year      =   {1996},
  author    =   {S.~L. Lauritzen}
}

@article{Chow68,
  author    =   {C.~K. Chow and C.~N. Liu},
  title     =   {Approximating discrete probability distributions with dependence trees},
  journal   =   IEEE_J_IT,
  month = mar,
  year      =   {1968},
  volume    =   {14},
  number    =   {3},
  pages     =   {462-467}
}

@ARTICLE{wainwright:GMs,
  title  =       {Graphical Models, Exponential Families and Variational Inference},
  author   =     {M. J. Wainwright and M. I. Jordan},
  journal =      {Foundations and Trends in Machine Learning},
  year    =  2008,
  volume = 1,
  number = "1-2",
  pages = "1-305"
}

@inproceedings{faceRec:Srinivas11,
  author    = "U. Srinivas and V. Monga and Y. Chen and T. D. Tran",
  title     = "Sparsity-based face recognition using discriminative graphical models",
  booktitle = "Proc. {IEEE} Asilomar Conf. on Signals, Systems and Computers",
  month     = nov,
  year      = 2011,
  pages     = {1204--1208},
  address   = "Pacific Grove, CA"
}

@ARTICLE{freund:Adaboost,
  AUTHOR  = {Yoav Freund and Robert E. Schapire},
  TITLE   = {A short introduction to boosting},
  JOURNAL = {Journal of Japanese Society for Artificial Intelligence},
  YEAR    = {1999},
  Volume  = {14},
  Number  = {5},
  PAGES =   {771-780},
  Month   = Sep
}

@article{Friedman97,
  author    =   {N. Friedman and D. Geiger and M. Goldszmidt},
  title     =   {Bayesian network classifiers},
  journal   =   {Machine Learning},
  month = nov,
  year      =   1997,
  volume    =   29,
  pages     =   "131-163"
}

@INPROCEEDINGS{Ho03,
    author = {J. Ho and M. Yang and J. Lim and K. Lee and D. Kriegman},
    title = {Clustering appearances of objects under varying illumination conditions},
    booktitle = ieee_cvpr,
    month = jun,
    year = {2003},
    address = "Madison, WI",
    pages = {11-18}
}

@book{Vapnik,
  author    =   {V.~N. Vapnik},
  title     =   {The nature of statistical learning theory},
  publisher =   {New York, USA: Springer},
  year      =   {1995}
}


@misc{GTechDatabase,
  title = {{\em The Georgia Tech Face Database}},
  url = {http://www.anefian.com/research/face_reco.htm}
}

@article{Liu01,
  author    =   {C. Liu and H. Wechsler},
  title     =   {A shape- and texture-based enhanced fisher classifier for face recognition},
  journal   =   IEEE_J_IP,
  month     =   apr,
  year      =   {2001},
  volume    =   {10},
  number    =   4,
  pages     =   {598-608}
}


@article{Zou07,
  author    =   {Jie Zou and Qiang Ji and G. Nagy},
  title     =   {A Comparative Study of Local Matching Approach for Face Recognition},
  journal   =   IEEE_J_IP,
  month     =   oct,
  year      =   {2007},
  volume    =   {16},
  number    =   {10},
  pages     =   {2617-2628}
}

@article{Wagner:robust_face,
  author    =   {A. Wagner and J. Wright and A. Ganesh and Z. Zhou and H. Mobahi and Y. Ma},
  title     =   {Towards a practical face recognition system: {R}obust alignment and illumination by sparse representation},
  journal   =   IEEE_J_PAMI,
  month     =   feb,
  year      =   {2012},
  volume    =   {34},
  number    =   {2},
  pages     =   {372-386}
}







@string{
    ap_acha = "Applied and Computational Harmonic Analysis"
}

@string{
    ieee_tcas2 = "IEEE Trans. Circuits and Systems---II: Analog and Digital Signal Processing"
}

@string{
    ieee_tsp = "IEEE Trans. Signal Process."
}

@string{
    ieee_tip = "IEEE Trans. Image Process."
}

@string{
    ieee_tit = "IEEE Trans. Inform. Theory"
}

@string{
    ieee_tnn = "IEEE Trans. Neural Networks"
}

@string{
    ieee_tcas = "IEEE Trans. Circuits Syst."
}

@string{
    ieee_tpami = "IEEE Trans. Pattern Anal. Machine Intell."
}

@string{
    ieee_tassp = "IEEE Trans. Acoustics, Speech, Signal Process."
}

@string{
    ieee_tgrs = "IEEE Trans. Geosci. Remote Sens."
}

@string{
    ieee_grsl = "IEEE Geosci. Remote Sens. Lett."
}

@string{
    ieee_pacrim = "Proc. IEEE Pacific Rim Conference on Communications,
      Computers and Signal Processing"
}

@string{
    ieee_icip = "Proc. IEEE Int. Conf. Image Process."
}


@string{
    ieee_icassp = "Proc. IEEE Int. Conf. Acoust., Speech, Signal Process."
}

@string{
    ieee_cvpr = "Proc. IEEE Conf. Comput. Vision Pattern Recogn."
}

@string{
    ieee_iscas = "Proc. IEEE Int. Symp. Circuits Syst."
}

@string{
    spie_vcip = "Proc. SPIE Visual Commun. Image Process."
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Publications
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{
    Wright_2009,
    author = "J. Wright and A. Y. Yang and A. Ganesh and S. Sastry and Y. Ma",
    title = "Robust Face Recognition via Sparse Representation",
    journal = ieee_tpami,
    volume = 31,
    number = 2,
    month = feb,
    year = 2009,
    pages = "210--227"
}

@article{wagner12:robustface,
    author = "A. Wagner and J. Wright and A. Ganesh and Z. Zhou and H. Mobahi and Y. Ma",
    title = "Toward a Practical Face Recognition System: {R}obust Alignment and Illumination by Sparse Representation",
    journal = ieee_tpami,
    volume = 34,
    number = 2,
    month = feb,
    year = 2012,
    pages = "372--386"
}

@article{
    Hang_2009,
    author = "X. Hang and F.-X. Wu",
    title = "Sparse Representation for Classification of Tumors Using Gene Expression Data",
    journal = "Journal of Biomedicine and Biotechnology",
    volume = 2009,
    year = 2009,
    note = "doi:10.1155/2009/403689"
}

@inproceedings{
    Pillai_2009,
    author = "J. K. Pillai and V. M. Patel and R. Chellappa",
    title = "Sparsity Inspired selection and recognition of iris images",
    booktitle = "Proc. IEEE Third Int. Conf. Biometrics: Theory, Applications and Systems",
    year = 2009,
    month = sep,
    pages = "1--6"
}

@inproceedings{
    Do_2009,
    author = "T. T. Do and Y. Chen and D. T. Nguyen and N. H. Nguyen and L. Gan and T. D. Tran",
    title = "Distributed compressed video sensing",
    booktitle = "Proc. {IEEE} Int. Conf. Image Process.",
    year = 2009,
    pages = "1393--1396",
    month = nov
}


@article{
    Basri_2003,
    author = "R. Basri and D. W. Jacobs",
    title = "Lambertian Reflectance and Linear Subspaces",
    journal = IEEE_J_PAMI,
    volume = 25,
    number = 2,
    month = feb,
    year = 2003,
    pages = "218--233"
}

@Article{
    CandesRob06,
    author = "E. Cand\`{e}s and J. Romberg and T. Tao",
    title =  "Robust uncertainty principles: Exact signal reconstruction from highly incomplete frequency information",
    journal = ieee_tit,
    volume =  52,
    number = 2,
    month = Feb,
    year = 2006,
    pages = "489--509"
}

@Article{
    Zhao_2003,
    author = "W. Zhao and R. Chellappa and P.~J. Phillips and A. Rosenfeld",
    title =  "Face Recognition: A Literature Survey",
    journal = "ACM Computing Surveys",
    volume =  35,
    number = 4,
    month = dec,
    year = 2003,
    pages = "399--458"
}

@inproceedings{
    Wagner_2009,
    author = "A. Wagner and J. Wright and A. Ganesh and Z. Zhou and Y. Ma",
    title = "Towards a practical face recognition system: Robust registration and illumination by sparse representation",
    booktitle = ieee_cvpr,
    pages = "597--604",
    month = jun,
    year = 2009
}

@inproceedings{
    Huang_2008,
    author = "J. Huang and X. Huang and D. Metaxas",
    title = "Simultaneous image transformation and sparse representation recovery",
    booktitle = ieee_cvpr,
    pages = "1--8",
    month = jun,
    year = 2008
}

@article{Tropp_2007,
  author = "J. Tropp and A. Gilbert",
  title =  "Signal recovery from random measurements via Orthogonal Matching Pursuit",
  journal = ieee_tit,
  volume =   53,
  number = 12,
  month =    dec,
  year =     2007,
  pages =    "4655--4666"
}

@article{Dai_2009,
  author = "W. Dai and O. Milenkovic",
  title =  "Subspace Pursuit for Compressive Sensing Signal Reconstruction",
  journal = ieee_tit,
    volume = 55,
    number = 5,
    month = may,
    year = 2009,
    pages = "2230--2249"
}

@inproceedings{
    Guo_2009,
    author = "Z. Guo and T. Wittman and S. Osher",
    title = "L1 unmixing and its application to hyperspectral image enhancement",
    booktitle = "Proc. SPIE Conf. on Algorithms and Technologies for Multispectral, Hyperspectral, and Ultraspectral Imagery XV.",
    volume = 7334,
    month = apr,
    year = 2009,
}

@article{GeBeKr01,
  author =  "A. S. Georghiades and P. N. Belhumeur and D. J. Kriegman",
  title =   "From Few to Many: Illumination Cone Models for Face Recognition under Variable Lighting and Pose",
  journal = IEEE_J_PAMI,
  month = jun,
  year =  2001,
  volume = 23,
  number = 6,
  pages= "643--660"
  }

@article{ARDatabase,
  author =  "A.~M. Martinez and R. Benavente",
  title =   {{The AR face database}},
  journal = "CVC Tech. Report",
  year =  1998,
  number = 24
  }

@article{Sirovitch_1987,
  author =  "L. Sirovitch and M. Kirby",
  title =   "Low-dimensional procedure for the characterization of human faces",
  journal = {J. Optical Soc. of Am. A},
  year =  1987,
  volume = 2,
  pages= "519--524"
  }


@article{Turk_1991,
    author = "M. Turk and A. Pentland",
    title = "Eigenfaces for recognition",
    journal = {J. Cogn. Neurosci.},
    volume = 3,
    number = 1,
    year = 1991,
    pages = "71-86"
}

@PHDTHESIS{Shashua_1992,
    AUTHOR = "A. Shashua",
    TITLE = {{Geometry and photometry in 3D visual recognition}},
    SCHOOL = "MIT",
    YEAR ="1992"}

@article{Belhumeur_1997,
    author = "P.~N. Belhumeur and J.~P. Hespanha and D.~J. Kriegman",
    title = "Eigenfaces vs. Fisherfaces: Recognition using class specific linear projection",
    journal = IEEE_J_PAMI,
    volume = 19,
    number = 7,
    year = 1997,
    pages = "711--720"
}

@article{Kittler98,
  author    =   {J. Kittler and M. Hatef and R.~P.~W. Duin and J. Matas},
  title     =   {On combining classifiers},
  journal   =   IEEE_J_PAMI,
  year      =   {1998},
  month     =   {Mar},
  volume    =   {20},
  number    =   {3},
  pages     =   {226-239}
}

@inproceedings{Chen_2009,
    author = "Y. Chen and T.~T. Do and T.~D. Tran",
    title = "Robust face recognition using locally adaptive sparse representation",
    booktitle = "Proc. {IEEE} Intl. Conf. Image Processing",
    year = 2010,
    pages = {1657--1660},
    month = sep
}

@article{Tan10,
  author    =   {V.~Y.~F. Tan and S. Sanghavi and J.~W. Fisher III and A.~S. Willsky},
  title     =   {Learning graphical models for hypothesis testing and classification},
  journal   =   {IEEE Trans. Signal Processing},
  year      =   {2010},
  volume    =   {58},
  number    =   {11},
  pages     =   {5481-5495},
  month     = 	{Nov}
}

@book{Lauritzen96,
  title     =   {{Graphical Models}},
  publisher =   {Oxford University Press, NY},
  year      =   {1996},
  author    =   {S.~L. Lauritzen}
}

@article{Chow68,
  author    =   {C.~K. Chow and C.~N. Liu},
  title     =   {Approximating discrete probability distributions with dependence trees},
  journal   =   IEEE_J_IT,
  year      =   {1968},
  volume    =   {14},
  number    =   {3},
  pages     =   {462-467}
}

@ARTICLE{wainwright:GMs,
  title  =       {Graphical Models, Exponential Families and Variational Inference},
  author   =     {M. J. Wainwright and M. I. Jordan},
  journal =      {Foundations and Trends in Machine Learning},
  year    =  2008,
  volume = 1,
  number = "1-2",
  pages = "1-305"
}

@inproceedings{faceRec:Srinivas11,
  author    = "U. Srinivas and V. Monga and Y. Chen and T. D. Tran",
  title     = "Sparsity-based face recognition using discriminative graphical models",
  booktitle = "Proc. {IEEE} Asilomar Conf. on Signals, Systems and Computers",
  year      = "2011"
}

@ARTICLE{freund:Adaboost,
  AUTHOR  = {Yoav Freund and Robert E. Shapire},
  TITLE   = {A short introduction to boosting},
  JOURNAL = {Journal of Japanese Society for Artificial Intelligence},
  YEAR    = {1999},
  Volume  = {14},
  Number  = {5},
  PAGES =   {771-780},
  Month   = {Sep.}}

@article{Friedman97,
  author    =   {N. Friedman and D. Geiger and M. Goldszmidt},
  title     =   {Bayesian network classifiers},
  journal   =   {Machine Learning},
  year      =   {1997},
  volume    =   {29},
  pages     =   {131-163}
}

@INPROCEEDINGS{Ho03,
    author = {J. Ho and M. Yang and J. Lim and K. Lee and D. Kriegman},
    title = {Clustering appearances of objects under varying illumination conditions},
    booktitle = ieee_cvpr,
    year = {2003},
    pages = {11--18}
}

@book{Vapnik,
  author    =   {V.~N. Vapnik},
  title     =   {The nature of statistical learning theory},
  publisher =   {New York, USA: Springer},
  year      =   {1995}
}


@misc{GTechDatabase,
  title = {{\em The Georgia Tech Face Database}},
  url = {http://www.anefian.com/research/face_reco.htm}
}

@article{Liu01,
  author    =   {C. Liu and H. Wechsler},
  title     =   {A shape- and texture-based enhanced fisher classifier for face recognition},
  journal   =   IEEE_J_IP,
  year      =   {2001},
  volume    =   {10},
  pages     =   {598--608}
}


@article{Zou07,
  author    =   {Jie Zou and Qiang Ji and G. Nagy},
  title     =   {A Comparative Study of Local Matching Approach for Face Recognition},
  journal   =   IEEE_J_IP,
  year      =   {2007},
  volume    =   {16},
  number    =   {10},
  pages     =   {2617--2628}
}

@article{Wagner:robust_face,
  author    =   {A. Wagner and J. Wright and A. Ganesh and Z. Zhou and H. Mobahi and Y. Ma},
  title     =   {Towards a practical face recognition system: {R}obust alignment and illumination by sparse representation},
  journal   =   IEEE_J_PAMI,
  year      =   {to appear}
}


@article{baraniuk10,
  author    =   {R.~G. Baraniuk and V. Cevher and M. Wakin},
  title     =   {Low-dimensional models for dimensionality reduction and signal recovery: {A} geometric perspective},
  journal   =   {{Proc. IEEE}},
  year      =   {2010},
  volume    =   {98},
  number    =   {6},
  pages     =   {959--971}
}

@article{chen:facerec,
  author    =   {Y. Chen and U. Srinivas and T.~T. Do and V. Monga and T.~D. Tran},
  title     =   {Discriminative local sparse representations for robust face recognition},
  journal   =   {{submitted to IEEE Trans. Image Processing}},
  year      =   {2011},
  month     =   nov
}

@article{
    Chen_2012_TGRS_KSR,
    author = "Y. Chen and N. M. Nasrabadi and T. D. Tran",
    title = "Hyperspectral Image Classification via Kernel Sparse Representation",
    journal = {{submitted to IEEE Trans. Geosci. Remote Sens.}},
    year = 2011,
    month = aug
}

@inproceedings{discGM:Srinivas11,
  author    = "Umamahesh Srinivas and Vishal Monga and Raghu G.~Raj",
  title     = "Automatic target recognition using discriminative graphical models",
  booktitle = "Proc. {IEEE} Intl. Conf. Image Processing",
  pages     = {33-36},
  month = sep,
  year      = 2011
}

@article{Chen_2011c,
    author = "Y. Chen and N. Nasrabadi and T.~D. Tran",
    title = "Hyperspectral image classification using dictionary-based sparse representation",
    journal = ieee_tgrs,
    volume = 49,
    number = 10,
    month = Oct,
    year = 2011,
    pages = "3973--3985"
}

@article{valls:compositeSVM,
    author = "G. Camps-Valls and L. Gomez-Chova and J. Munoz-Mari and J. Vila-Frances and J. Calpe-Maravilla",
    title = {{Composite kernels for hyperspectral image classification}},
    journal = {{IEEE} Geosci. Remote Sensing Letters},
    volume = 3,
    number = 1,
    month = Jan,
    year = 2006,
    pages = "93--97"
}


@article{Donoho_2006a,
    author = "D. L. Donoho",
    title = "Compressed Sensing",
    journal = ieee_tit,
    volume = 52,
    number = 4,
    year = 2006,
    month = apr,
    pages = "1289--1306"
}

@article{
    Donoho_2006b,
    author = "D. L. Donoho",
    title = "For most large underdetermined systems of linear equations the minimal $l_1$-norm solution is also the sparsest solution",
    journal = "Comm. Pure and Applied Math.",
    volume = 59,
    number = 6,
    year = 2006,
    pages = "797--829"
}

@article{Bruckstein_2009,
  author = "A. M. Bruckstein and D. L. Donoho and M. Elad",
  title =  "From Sparse Solutions of Systems of Equations to Sparse Modeling of Signals and Images ",
  journal = "SIAM Review",
    volume = 51,
    number = 1,
    year = 2009,
    pages = "34--81"
}

@inproceedings{
    Elhamifar_2009,
    author = "E. Elhamifar and R. Vidal",
    title = "Sparse subspace clustering",
    booktitle = ieee_cvpr,
    pages = "2790--2797",
    month = jun,
    year = 2009
}

@inproceedings{
    Do_2008b,
    author = "T. T. Do and L. Gan and N. H. Nguyen and T. D. Tran",
    title = "Sparsity adaptive matching pursuit algorithm for practical compressed sensing",
    booktitle = "Proc. IEEE Asilomar Conf. on Signals, Systems, and Computers",
    month = oct,
    year = 2008,
    pages = "581-587",
    address = "Pacific Grove, CA"
}


@article{
    Pillai_2011,
    author = "J. K. Pillai and V. M. Patel and R. Chellappa and N. Ratha",
    title = "Secure and robust iris recognition using Sparse Representations and Random Projections",
    journal = ieee_tpami,
    volume = 33,
    number = 9,
    month = sep,
    year = 2011,
    pages = "1877--1893"
}

@article{Blumensath_2009,
  author = "T. Blumensath and M. E. Davies",
  title =  "Sampling Theorems for Signals From the Union of Finite-Dimensional Linear Subspaces",
  journal = ieee_tit,
    volume = 55,
    year = 2009,
    pages = "1872--1882"
}

@article{
    Ji_2008,
    author = "S. Ji and Y. Xue and L. Carin",
    title = "Bayesian Compressive Sensing ",
    journal = ieee_tsp,
    volume = 56,
    number = 6,
    month = jun,
    year = 2008,
    pages = "2346--2356"
}


@BOOK{Mallat,
  AUTHOR =       {S. Mallat},
  TITLE =        {A Wavelet Tour of Signal Processing, Third Edition},
  PUBLISHER =    {Academic Press},
  YEAR =         {2008},
}

@INPROCEEDINGS{Li_2011,
author="Ce Li and Zhenjun Han and Qixiang Ye and Jianbin Jiao",
title="Abnormal Behavior Detection via Sparse Reconstruction Analysis of Trajectory",
booktitle="Sixth IEEE Int. Conf. Image and Graphics",
year=2011,
month="Aug.",
pages="807-810"
}

@ARTICLE{Wang_2009,
author={Xiaogang Wang and Xiaoxu Ma and W.~E.~L. Grimson},
journal={IEEE Trans. Pattern Anal. Machine Intell.},
title={Unsupervised Activity Perception in Crowded and Complicated Scenes Using Hierarchical {B}ayesian Models},
year={2009},
month={Mar.},
volume={31},
number={3},
pages={539-555},
keywords={complicated scenes;crowded traffic scenes;dual hierarchical Dirichlet processes model;hierarchical Bayesian models;hierarchical Dirichlet process mixture model;language models;latent dirichlet allocation mixture model;motion segmentation;multiagent interactions;train station scenes;unsupervised activity perception;unsupervised learning framework;video clips;video sequence;visual features;visual surveillance tasks;Bayes methods;image segmentation;learning (artificial intelligence);video surveillance;Algorithms;Artificial Intelligence;Bayes Theorem;Computer Simulation;Humans;Image Enhancement;Image Interpretation, Computer-Assisted;Models, Biological;Models, Statistical;Pattern Recognition, Automated;Reproducibility of Results;Sensitivity and Specificity;Subtraction Technique;Whole Body Imaging;},
doi={10.1109/TPAMI.2008.87},
ISSN={0162-8828}}

@INPROCEEDINGS{Han_2004,
author={Mei Han and Wei Xu and Hai Tao and Yihong Gong},
booktitle={Proc. IEEE Conf. Computer Vision and Pattern Recognition},
title={An algorithm for multiple object trajectory tracking},
year={2004},
month={Jun.},
pages={864--871},
keywords={ Hidden Markov model; MAP solution; joint state observation probability; likelihood computation; maximum a posteriori solution; multiobject configuration; multiple object trajectory tracking; object detection map; object state estimation; observation model; optimal state sequence estimation; pixel wise object detection scores; probabilistic framework; temporal distractions; hidden Markov models; maximum likelihood sequence estimation; object detection; probability; state estimation; tracking;},
doi={10.1109/CVPR.2004.1315122},
ISSN={1063-6919 }}

@ARTICLE{Vaswani_2005,
author={N. Vaswani and A.~K. Roy-Chowdhury and R. Chellappa},
journal={IEEE Trans. Image Processing},
title={Shape activity: a continuous-state {HMM} for moving/deforming shapes with application to abnormal activity detection},
year={2005},
month={Oct.},
volume={14},
number={10},
pages={1603-1616},
keywords={abnormal activity detection;activity recognition;co-occurrence statistics;continuous-state hidden Markov model;dynamic Bayesian networks;hidden-state vector;particle filtering;scaled Euclidean motion parameter;shape deforming;belief networks;filtering theory;hidden Markov models;image motion analysis;image recognition;statistics;Algorithms;Artificial Intelligence;Computer Simulation;Humans;Image Enhancement;Image Interpretation, Computer-Assisted;Information Storage and Retrieval;Markov Chains;Models, Biological;Models, Statistical;Movement;Pattern Recognition, Automated;Subtraction Technique;Video Recording;},
doi={10.1109/TIP.2005.852197},
ISSN={1057-7149}}


@article{Huttenlocher_2005,
    author = "P.~F. Felzenszwalb and D.~P. Huttenlocher",
    title = "Pictorial structures for object recognition",
    journal = {{Int. Journal of Computer Vision}},
    volume = 61,
    number = 1,
    month = Jan,
    year = 2005,
    pages = "55--79"
}

@article{Fischler_1973,
    author = "M.~A. Fischler and R.~A. Elschlager",
    title = "The representation and matching of pictorial structures",
    journal = {{IEEE Trans. Computer}},
    volume = 22,
    number = 1,
    month = Jan,
    year = 1973,
    pages = "67--92"
}


@inproceedings{Stauffer_1999,
    author = "C. Stauffer and W. Grimson",
    title = "Adaptive background mixture models for real-time tracking",
    booktitle = {{Proc. IEEE Conf. on CVPR}},
    year = 1999,
    pages = "246--252"
}


@inproceedings{Bradski_1998,
    author = "G. Bradski",
    title = "Realtime face and object tracking as a component of a perceptual user interface",
    booktitle = {{Proc. IEEE Workshop on Applications of Computer Vision}},
    year = 1998,
    pages = "214--219"
}

@article{Papanikolopoulos_1993,
    author = "N. Papanikolopoulos and P. Khosla and T. Kanade",
    title = "Visual tracking of a moving target by a camera mounted on a robot: A combination of control and vision",
    journal = {{IEEE Trans. Robotics and Automation}},
    volume = 9,
    year = 1993,
    pages = "14--35"
}

@inproceedings{Roberts_1965,
    author = "L.~G. Roberts",
    title = "Machine perception of 3-{D} solids",
    booktitle = {{Optical and Electro-optical Information Processing}},
    year = 1965,
    pages = "159--197"
}

@article{Ayache_1986,
    author = "N.~J. Ayache and O.~D. Faugeras",
    title = "Hyper: A new approach for the recognition and positioning of two-dimensional objects",
    journal = {{IEEE Trans. Pattern Anal. Machine Intell.}},
    volume = 8,
    number = 1,
    month = Jan,
    year = 1986,
    pages = "44--54"
}

@article{fischler_1985,
    author = "M.~A. Fischler and R.~C. Bolles",
    title = "Random sample consensus: A paradigm for model fitting with applications to image analysis and automated cartography",
    journal = {{Communications of the ACM}},
    volume = 24,
    number = 6,
    month = Jun,
    year = 1981,
    pages = "381--395"
}


@article{lamdan_1990,
    author = "Y. Lamdan and J.~T. Schwartz and H.~J. Wolfson",
    title = "Affine invariant model-based object recognition",
    journal = {{IEEE Trans. Robotics and Automation}},
    volume = 6,
    number = 5,
    year = 1990,
    pages = "578--589"
}

@article{huttenlocher_1993,
    author = "D.~P. Huttenlocher and G.~A. Klanderman and W.~J. Rucklidge",
    title = "Comparing images using the Hausdorff distance",
    journal = {{IEEE Trans. Pattern Anal. Machine Intell.}},
    volume = 15,
    number = 9,
    year = 1993,
    month = Sep,
    pages = "850--863"
}

@inproceedings{Lowe99,
    Author  = {D.~G. Lowe},
    Title   = {Object recognition from local scale-invariant features},
    Booktitle = {Int. Conf. Computer Vision},
    Year    = {1999},
    Month   = {September}}

@article{viola_2004,
    author = "Paul Viola and Michael Jones",
    title = "Robust real-time object detection",
    journal = {{Int. Journal of Computer Vision}},
    volume = 57,
    number = 2,
    year = 2004,
    pages = "137--154"
}

@article{cootes_2001,
    author = "T.~F. Cootes and G.~J. Edwards and C.~J. Taylor",
    title = "Active appearance models",
    journal = {{IEEE Trans. Pattern Anal. Machine Intell.}},
    volume = 23,
    number = 6,
    year = 2001,
    pages = "681--685"
}

@article{cootes_1995,
    author = "T.~F. Cootes and C.~J. Taylor and D.~H. Cooper and J. Graham ",
    title = "Active shape models - their training and application",
    journal = {{Computer Vision and Image Understanding}},
    volume = 61,
    year = 1995,
    pages = "38--59"
}

@article{rosenfeld_1976,
    author = "A. Rosenfeld and R.~A. Hummel and S.~W. Zucker",
    title = "Scene labelling by relaxation operations",
    journal = {{IEEE Trans. Systems, Man and Cybernetics}},
    volume = 6,
    year = 1976,
    pages = "420--433"
}

@article{feldman_1974,
    author = "J.~A. Feldman and Y. Yakimovsky",
    title = "Decision theory and artificial intelligence: A semantics-based region analyzer",
    journal = {{Artifical Intelligence}},
    volume = 5,
    number = 4,
    year = 1974,
    pages = "349--371"
}

@inproceedings{grauman_2005,
  author    =   {Kristen Grauman and Trevor Darrel},
  title     =   {The Pyramid Match Kernel: Discriminative Classification with Sets of Image Features},
  booktitle =   {{Proc. IEEE Int. Conf. Computer Vision}},
  year      =   {2005},
  month     =   oct,
  pages     =   {1458--1465}
}



@article{Johnson_1996,
    author = "N. Johnson and D. Hogg",
    title = "Learning the distribution of object trajectories for event recognition",
    journal = {Image Vision Computing},
    volume = 3,
    number = 1,
    year = 1996,
    pages = "609--615"
}

@inproceedings{Owens_2000,
    author = "J. Owens and A. Hunter",
    title = "Application of the self-organizing map to trajectory classification",
    booktitle = {{IEEE Int. Workshop on Visual Surveillance}},
    year = 2000
}

@article{Hu_2006,
    author = "W. Hu and X. Xiao and Z. Fu and D. Xie and T. Tan and S.~J. Maybank",
    title = "A system for learning statistical motion patterns",
    journal = {{IEEE Trans. Pattern Anal. Machine Intell.}},
    year = 2006,
    pages = "1450--1464"
}

@article{Makris_2005,
    author = "D. Makris and T. Ellis",
    title = "Learning semantic scene models from observing activity in visual surveillance",
    journal = {{IEEE Trans. Systems, Man, and Cybernetics}},
    year = 2005,
    pages = "397--408"
}

@inproceedings{Wang_2008,
    author = "X. Wang and E. Grimson",
    title = "Trajectory analysis and semntic region modeling using a nonparametric {B}ayesian model",
    booktitle = {{IEEE Conf. Computer Vision and Pattern Recognition}},
    year = 2008
}

@article{srinivas:hsiclass,
  author    =   {U. Srinivas and Y. Chen and V. Monga and N.~M. Nasrabadi and T.~D. Tran},
  title     =   {Exploiting sparsity in hyperspectral image classification via graphical models},
  journal   =   {{submitted to IEEE Geoscience and Remote Sensing Letters}},
  year      =   {2011},
  month     =   dec
}


@inproceedings{srinivas:hsidet,
  author    =   {U. Srinivas and Y. Chen and V. Monga and N.~M. Nasrabadi and T.~D. Tran},
  title     =   {Discriminative Graphical Models For Sparsity-Based Hyperspectral Target Detection},
  booktitle =   {{submitted to IEEE Int. Geoscience and Remote Sensing Symposium}},
  year      =   {2012},
  month     =   jan
}

@inproceedings{chen:mmsp,
  author    =   {S. Chen and V. Monga and P. Moulin},
  title     =   {Meta-classifiers for multi-modal document classification},
  booktitle =   {{IEEE Int. Workshop on Multimedia Signal Processing}},
  year      =   {2009},
  month     =   oct
}


@article{Nguyen_2012_PR,
    author = "N. H. Nguyen and N. M. Nasrabadi and T. D. Tran",
    title = "Joint Kernel Sparse Representation for Classification with Applications for Personnel Detection",
    journal = {{submitted to Pattern Recognition}},
    month = feb,
    year = 2012
}


@book{Scholkopf_2001,
    author = "B. Sch{\"o}lkopf and A. J. Smola",
    title = "Learning with Kernels: Support Vector Machines, Regularization, Optimization, and Beyond",
    publisher = "The MIT Press",
    year = 2001
}

@inproceedings{Gao_2010,
    author = "S. Gao and I. W. Tsang and L.-T. Chia",
    title = "Kernel Sparse Representation for Image Classification and Face Recognition",
    booktitle = "Proc. 11th European Conf. Computer Vision",
    volume = 6314,
    month = sep,
    year = 2010
}

@inproceedings{Yuan_2010,
    author = "X.-T. Yuan and S. Yan",
    title = "Visual classification with multi-task joint sparse representation",
    booktitle = ieee_cvpr,
    month = jun,
    year = 2010,
    address = "San Francisco, CA"
}

@article{Vincent_2002,
    author = "P. Vincent and Y. Bengio",
    title = "Kernel Matching Pursuit",
    journal = "Machine Learning",
    volume = 48,
    year = 2002,
    pages = "165--187"
}

@article{Guigue_2006,
    author = "V. Guigue and A. Rakotomamonjy and S. Canu",
    title = "Kernel Basis Pursuit",
    journal = "New Methods in Machine Learning",
    year = 2006,
    volume = 20,
    number = 6,
    pages = "757--774"
}


@article{Roth_2004,
    author = "V. Roth",
    title = "The Generalized {LASSO}",
    journal = ieee_tnn,
    volume = 15,
    year = 2004,
    pages = "16-28"
}

@article{Camps-Valls_2006,
    author = "G. Camps-Valls and L. Gomez-Chova and J. Mu{\~{n}}oz-Mar\'{i} and J. Vila-Franc\'{e}s and J. Calpe-Maravilla",
    title =  "Composite kernels for hyperspectral image classification",
    journal = ieee_grsl,
    volume =  3,
    number = 1,
    month = Jan,
    year = 2006,
    pages = "93--97"
}


@book{Tychonoff_1977,
    author = "A.~N. Tikhonov and V.~Y. Arsenin",
    title = "Solution of Ill-posed Problems",
    publisher = "Winston \& Sons",
    year = 1977
}


%% Block sparsity
@article{
    Eldar_2009,
    author = "Y. C. Eldar and M. Mishali",
    title = "Robust Recovery of Signals From a Structured Union of Subspaces",
    journal = ieee_tit,
    volume = 55,
    number = 11,
    year = 2009,
    month = nov,
    pages = "5302--5316"
}

@article{Stojnic_2009,
    author = "M. Stojnic and F. Parvaresh and B. Hassibi",
    title =  "On the reconstruction of block-sparse signals with an optimal number of measurements",
    journal = ieee_tsp,
    volume =  57,
    number = 8,
    month = aug,
    year = 2009,
    pages = "3075--3085"
}

@techreport{Baron05distributedcompressed,
    author = {Dror Baron and Michael B. Wakin and Marco F. Duarte and Shriram Sarvotham and Richard G. Baraniuk},
    title = {Distributed compressed sensing},
    year = {2005}
}


%% Connected-tree for wavelets
@article{Shapiro_1993,
    author = "J. Shapiro",
    title = "Embedded image coding using zerotrees of wavelet coefficients",
    journal = ieee_tsp,
    volume = 41,
    number = 12,
    month = dec,
    year = 1993,
    pages = "3445--3462"
}

@article{baraniuk94,
    author = "R.~G. Baraniuk and D.~L. Jones",
    title = "A signal-dependent time-frequency representation: {F}ast algorithm for optimal kernel design",
    journal = ieee_tsp,
    volume = 42,
    number = 1,
    month = jan,
    year = 1994,
    pages = "134--146"
}

@article{crouse98,
    author = "M.~S. Crouse and R.~D. Nowak and R.~G. Baraniuk",
    title = "Wavelet-based statistical signal processing using hidden {M}arkov models",
    journal = ieee_tsp,
    volume = 46,
    number = 4,
    month = apr,
    year = 1998,
    pages = "886--902"
}

@article{romberg01,
    author = "J.~K. Romberg and H. Choi and R.~G. Baraniuk",
    title = "Bayesian tree-structured image modeling using wavelet-domain hidden {M}arkov models",
    journal = ieee_tip,
    volume = 10,
    number = 7,
    month = jul,
    year = 2001,
    pages = "1056--1068"
}

@article{portilla03,
    author = "J. Portilla and V. Strela and M.~J. Wainwright and E.~P. Simoncelli",
    title = "Image denoising using a scale mixture of {G}aussians in the wavelet domain",
    journal = ieee_tip,
    volume = 12,
    number = 11,
    month = nov,
    year = 2003,
    pages = "1338--1351"
}

@inproceedings{cevher09:nips,
    author = "V. Cevher",
    title = "Learning with compressible priors",
    booktitle = "Proc. Neural Information Processing Systems",
    year = 2009,
    month = dec,
    pages = "261--269"
}

%% Dictionary learning
@article{rubinstein10,
    author = "R. Rubinstein and A.~M. Bruckstein and M. Elad",
    title = "Dictionaries for sparse representation modeling",
    journal = {{Proc. IEEE}},
    volume = 98,
    number = 6,
    month = jun,
    year = 2010,
    pages = "1045--1057"
}

@article{aharon06:ksvd,
  author =  "M. Aharon and M. Elad and A. M. Bruckstein",
  title =   {{K-SVD: An algorithm for designing overcomplete dictionaries for sparse representation}},
  journal = ieee_tsp,
  month = nov,
  year =  2006,
  volume = 54,
  number = 11,
  pages= "4311--4322"
}

@article{elad06,
  author =  "M. Elad and M. Aharon",
  title =   "Image denoising via sparse and redundant representations over learned dictionaries",
  journal = ieee_tip,
  month = dec,
  year =  2006,
  volume = 15,
  number = 12,
  pages= "3736--3745"
}

@article{olshausen96,
  author =  "B.~A. Olshausen and D.~J. Field",
  title =   "Emergence of simple-cell receptive field properties by learning a sparse code for natural images",
  journal = "Nature",
  year =  1996,
  volume = 381,
  number = 6583,
  pages= "607--609"
}

@inproceedings{engan99:icassp,
    author = "K. Engan and S.~O. Aase and J. Hakon Husoy",
    title = "Method of optimal directions for frame design",
    booktitle = {{Proc. IEEE Int. Conf. Acoust., Speech, Signal Process.}},
    year = 1999,
    vol = "5",
    pages = "2443--2446"
}

@inproceedings{thiagarajan11:asilomar,
    author = "J.~J. Thiagarajan and A. Spanias",
    title = "Learning dictionaries for local sparse coding in image classification",
    booktitle = {{Proc. IEEE Asilomar Conf.}},
    year = 2011
}

@techreport{rodriguez08,
    author = {F. Rodriguez and G. Sapiro},
    title = {Sparse representations for image classification: {L}earning discriminative and reconstructive non-parametric dictionaries},
    institution = {U. Minnesota},
    year = {2008}
}

@inproceedings{zhang10:dksvd,
    author = "Q. Zhang and B. Li",
    title = "Discriminative {K}-{SVD} for dictionary learning in face recognition",
    booktitle = ieee_cvpr,
    year = 2010,
    pages = "2691--2698"
}

%% Spike-and-slab prior
@article{george93:spike,
  author    =   {E.~I. George and R.~E. McCulloch},
  title     =   {{Variable selection via Gibbs sampling}},
  journal   =   {J. Amer. Statist. Assoc.},
  year      =   {1993},
  volume    =   {88},
  pages     =   {881--889}
}


@article{chipman96:spike,
  author    =   {H. Chipman},
  title     =   {{Bayesian variable selection with related predictors}},
  journal   =   {Canad. J. Statist.},
  year      =   {1996},
  volume    =   {24},
  pages     =   {17--36}
}

@article{carvalho08:spike,
  author    =   {C. Carvalho and J. Chang and J. Lucas and Q. Wang and J. Nevins and M. West},
  title     =   {{High-dimensional sparse factor modelling: Applications in gene expression genomics}},
  journal   =   {J. Amer. Statist. Assoc.},
  year      =   {2008},
  volume    =   {103},
  pages     =   {1438--1456}
}

%% GMs on sparse coefficients
@inproceedings{cevher08:nips,
    author = "V. Cevher and M.~F. Duarte and C. Hegde and R.~G. Baraniuk",
    title = "Sparse signal recovery using {M}arkov random fields",
    booktitle = "Proc. Neural Information Processing Systems",
    year = 2008,
    month = dec,
    pages = "257--264"
}

@inproceedings{wainwright00:nips,
    author = "M.~J. Wainwright and E.~P. Simoncelli",
    title = "Scale mixtures of {G}aussians and the statistics of natural images",
    booktitle = "Proc. Neural Information Processing Systems",
    year = 2000,
    month = dec,
    pages = "855--861"
}


@inproceedings{
    Boser_1992,
    author = "B. E. Boser and I. M. Guyon and V. N. Vapnik",
    title = "A training algorithm for optimal margin classifiers",
    booktitle = "Proc. Fifth Annual Workshop on Computational Learning Theory",
    year = 1992,
    pages = "144--152",
    address = {Pittsburgh, PA, USA},
    publisher = {ACM},
}

@article{
  Aizerman_1964,
  author    =   "M. A. Aizerman and E. M. Braverman and L. I. Rozonoer",
  title     =   "Theoretical foundations of the potential function method in pattern recognition learning",
  journal   =   "Automation and Remote Control",
  year      =   1964,
  volume    =   25,
  number    =   6,
  pages     =   "821--837"
}




@string{
    ap_acha = "Applied and Computational Harmonic Analysis"
}

@string{
    ieee_tcas2 = "IEEE Trans. Circuits and Systems---II: Analog and Digital Signal Processing"
}

@string{
    ieee_tsp = "IEEE Trans. Signal Process."
}

@string{
    ieee_tip = "IEEE Trans. Image Process."
}

@string{
    ieee_tit = "IEEE Trans. Inform. Theory"
}

@string{
    ieee_tnn = "IEEE Trans. Neural Networks"
}

@string{
    ieee_tcas = "IEEE Trans. Circuits Syst."
}

@string{
    ieee_tpami = "IEEE Trans. Pattern Anal. Machine Intell."
}

@string{
    ieee_tassp = "IEEE Trans. Acoust., Speech, Signal Process."
}

@string{
    ieee_tgrs = "IEEE Trans. Geosci. Remote Sens."
}

@string{
    ieee_grsl = "IEEE Geosci. Remote Sens. Lett."
}


@string{
    ieee_icip = "Proc. IEEE Int. Conf. Image Process."
}


@string{
    ieee_icassp = "Proc. IEEE Int. Conf. Acoust., Speech, Signal Process."
}

@string{
    ieee_cvpr = "Proc. IEEE Conf. Comput. Vision Pattern Recogn."
}

@string{
    ieee_iscas = "Proc. IEEE Int. Symp. Circuits Syst."
}

@string{
    spie_vcip = "Proc. SPIE Visual Commun. Image Process."
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Publications
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{babacan:tip10,
    author 	= {S. Derin Babacan and Rafael Molina and Aggelos K. Katsaggelos},
    title 	= {Bayesian Compressive Sensing Using {L}aplace Priors},
    journal = ieee_tip,
    volume 	= 19,
    number 	= 1,
    month 	= jan,
    year 	= 2010,
    pages 	= {53--63}
}


@article{baraniuk_modelbasedcs:tit10,
    author 	= {R.~G. Baraniuk and V. Cevher and M.~F. Duarte and C. Hegde},
    title 	= {Model-based compressive sensing},
    journal = ieee_tit,
    volume 	= 56,
    number 	= 4,
    year 	= 2010,
    month 	= apr,
    pages 	= {1982--2001}
}


@article{bruckstein:siam09,
	author 	= {A.~M. Bruckstein and D.~L. Donoho and M. Elad},
	title 	= {From Sparse Solutions of Systems of Equations to Sparse Modeling of Signals and Images},
	journal = {SIAM Review},
	volume 	= 51,
	number 	= 1,
	year 	= 2009,
    pages 	= {34--81}
}


@article{ji_bcs:tsp08,
    author 	= {S. Ji and Y. Xue and L. Carin},
    title 	= {Bayesian compressive sensing},
    journal = ieee_tsp,
    volume 	= 56,
    number 	= 6,
    month 	= jun,
    year 	= 2008,
    pages 	= {2346--2356}
}


@article{ji_mcs:tsp09,
    author 	= {S. Ji and D. Dunson and L. Carin},
    title 	= {Multitask compressive sensing},
    journal = ieee_tsp,
    volume 	= 57,
    number 	= 1,
    month 	= jan,
    year 	= 2009,
    pages 	= {92--106}
}


@article{carin_spike:tsp09,
    author 	= {L. He and L. Carin},
    title 	= {Exploiting Structure in Wavelet-based {B}ayesian compressive sensing},
    journal = ieee_tsp,
    volume 	= 57,
    number 	= 9,
    month 	= sep,
    year 	= 2009,
    pages 	= {3488--3497}
}


@book{taubman_jpeg:01,
  title     =   {{JPEG 2000: Image Compression Fundamentals, Standards and Practice}},
  publisher =   {Kluwer Academic, Norwell, MA},
  year      =   {2001},
  author    =   {D.~S. Taubman and M.~W. Marcellin}
}


@article{lustig_mri:mrm07,
    author 	= {M. Lustig and D.~L. Donoho and J.~L. Pauly},
    title 	= {Sparse {MRI}: The Application of Compressed Sensing for Rapid {MR} Imaging},
    journal = {Magnetic Resonance in Medicine},
    volume 	= 58,
    year 	= 2007,
    pages 	= {1182--1195}
}


@article{donoho:cpam06,
    author  = {D.~L. Donoho},
    title   = {For most large underdetermined systems of linear equations the minimal $l_1$-norm solution is also the sparsest solution},
    journal = {Comm. Pure Appl. Math.},
    volume  = 59,
    number  = 6,
    year    = 2006,
    pages   = {797--829}
}

@article{tibshirani_lasso:jrss96,
    author  = {R. Tibshirani},
    title   = {Regression shrinkage and selection via the {LASSO}},
    journal = {J. Royal Statistical Soc. B},
    volume  = 58,
    number  = 1,
    year    = 1996,
    pages   = {267--288}
}

@article{aharon_ksvd:tsp06,
    author  =  {M. Aharon and M. Elad and A.~M. Bruckstein},
    title   = {{K-SVD}: An algorithm for designing overcomplete dictionaries for sparse representation},
    journal = ieee_tsp,
    month   = nov,
    year    = 2006,
    volume  = 54,
    number  = 11,
    pages   = {4311--4322}
}

@article{rubinstein:pieee10,
    author  = {R. Rubinstein and A.~M. Bruckstein and M. Elad},
    title   = {Dictionaries for sparse representation modeling},
    journal = {{Proc. IEEE}},
    volume  = 98,
    number  = 6,
    month   = jun,
    year    = 2010,
    pages   = {1045--1057}
}


@article{wright:pami09,
    author  = {J. Wright and A.~Y. Yang and A. Ganesh and S. Sastry and Y. Ma},
    title   = {Robust Face Recognition via Sparse Representation},
    journal = ieee_tpami,
    volume  = 31,
    number  = 2,
    month   = feb,
    year    = 2009,
    pages   = {210--227}
}


@article{olshausen:vr97,
    author  = {B. Olshausen and D. Field},
    title   = {Sparse Coding with an Overcomplete Basis Set: A Strategy Employed by {V}1?},
    journal = {Vision Research},
    volume  = 37,
    year    = 1997,
    pages   = {3311--3325}
}


@article{cevher:spm10,
  author    =   {V. Cevher and P. Indyk and L. Carin and R.~G. Baraniuk},
  title     =   {Sparse signal recovery and acquisition with graphical models},
  journal   =   {IEEE Signal Process. Mag.},
  year      =   {2010},
  volume    =   {27},
  number    =   {6},
  pages     =   {92--103}
}

@article{tipping:jmlr01,
  author    =   {M. Tipping},
  title     =   {Sparse {B}ayesian learning and the relevance vector machine},
  journal   =   {J. Mach. Learn. Res.},
  year      =   {2001},
  pages     =   {211--244}
}


@article{duarte:tsp11,
  author    = {M. Duarte and Y.~C. Eldar},
  title     = {Structured compressed sensing: {F}rom theory to applications},
  journal   = ieee_tsp,
  year      = {2011},
  volume    = {59},
  number    = {9},
  month     = sep,
  pages     = {4053--4085}
}


@article{candes:tit06,
    author  = {E. Cand\`{e}s and J. Romberg and T. Tao},
    title   = {Robust uncertainty principles: Exact signal reconstruction from highly incomplete frequency information},
    journal = ieee_tit,
    volume  = 52,
    number  = 2,
    month   = feb,
    year    = 2006,
    pages   = {489--509}
}


%% Spike-and-slab prior
@article{ishwaran_spike:as05,
  author    =   {H. Ishwaran and J.~S. Rao},
  title     =   {{Spike and slab variable selection: Frequentist and Bayesian strategies}},
  journal   =   {Ann. Stat.},
  year      =   {2005},
  volume    =   {33},
  pages     =   {730--773}
}

@article{george_spike:jasa93,
  author    =   {E.~I. George and R.~E. McCulloch},
  title     =   {{Variable selection via Gibbs sampling}},
  journal   =   {J. Amer. Statist. Assoc.},
  year      =   {1993},
  volume    =   {88},
  pages     =   {881--889}
}


@article{chipman_spike:cjs96,
  author    =   {H. Chipman},
  title     =   {Bayesian variable selection with related predictors},
  journal   =   {Canad. J. Statist.},
  year      =   {1996},
  volume    =   {24},
  pages     =   {17--36}
}

@article{carvalho_spike:jasa08,
    author    =   {C. Carvalho and J. Chang and J. Lucas and Q. Wang and J. Nevins and M. West},
    title     =   {{High-dimensional sparse factor modelling: Applications in gene expression genomics}},
    journal   =   {J. Amer. Statist. Assoc.},
    year      =   {2008},
    volume    =   {103},
    pages     =   {1438--1456}
}

@inproceedings{titsias:nips11,
    author      = {Michalis K. Titsias and Miguel L\'{a}zaro-Gredilla},
    title       = {Spike and Slab Variational Inference for Multi-Task and Multiple Kernel Learning},
    booktitle   = "Adv. Neural Inform. Process. Syst. 25",
    year        = 2011
}

@article{carvalho:jmlr09,
  author    =   {Carlos M. Carvalho and Nicholas G. Polson and James G. Scott},
  title     =   {Handling Sparsity via the Horseshoe},
  journal   =   {{J. Mach. Learn. Res., W$\&$CP 5 (AIStats)}},
  year      =   2009
}


@article{yen:as11a,
  author    =   {Tso-Jung Yen},
  title     =   {A majorization-minimization approach to variable selection using spike and slab priors},
  journal   =   {Ann. Stat.},
  year      =   2011,
  volume    =   {39},
  number    =   {3},
  pages     =   {1748--1775}
}


@article{zou:jrss05,
  author    =   {Hui Zou and Trevor Hastie},
  title     =   {Regularization and variable selection via the elastic net},
  journal   =   {J. R. Statist. Soc. B},
  year      =   2005,
  volume    =   {67},
  number    =   {2},
  pages     =   {301--320}
}

@article{bach_spams:ftml12,
  author    =   {F. Bach and R. Jenatton and J. Mairal and G. Obozinski},
  title     =   {Optimization with Sparsity-Inducing Penalties},
  journal   =   {Foundations and Trends in Machine Learning},
  year      =   2012,
  volume    =   {4},
  number    =   {1},
  pages     =   {1--106}
}

@misc{aviris,
    title   = {{AVIRIS NW Indiana's Indian Pines 1992 Data Set}},
    url     = {http://cobweb.ecn.purdue.edu/biehl/MultiSpec/documentation.html}
}


@article{pillai:pami11,
    author  = {J.~K. Pillai and V.~M. Patel and R. Chellappa and N.~K. Ratha},
    title   = {Secure and robust iris recognition using random projections and sparse representations},
    journal = ieee_tpami,
    volume  = 33,
    number  = 9,
    month   = sep,
    year    = 2011,
    pages   = {1877--1893}
}

@inproceedings{gualtieri:spie98,
    author      = {J.~A. Gualtieri and R.~F. Cromp},
    title       = {Support vector machines for hyperspectral remote sensing classification},
    booktitle   = {Proc. SPIE},
    volume      = {3584},
    pages       = {221--232},
    month       = jan,
    year        = 1998
}

@article{madabhushi:rbe09,
    title   =   {Histopathological image analysis: a review},
    author  =   {Metin N.~Gurcan and Laura E.~Boucheron and Ali Can and Anant Madabhushi and Nasir M.~Rajpoot and Bulent Yener},
    journal =   {IEEE Rev. Biomed. Eng.},
    year    =   2009,
    volume  =   2,
    pages   =   {147--171}
}

@article{orlov_wndcharm:prl08,
    author  = {Nikita Orlov and Lior Shamir and Tomasz Macura and Josiah Johnston and D. Mark Eckley and Ilya G. Goldberg},
    title   = {{WND-CHARM: Multi-purpose image classification using compound image transforms}},
    journal = {Pattern Recogn. Lett.},
    volume  = 29,
    number  = 11,
    year    = 2008,
    pages   = {1684--1693}
}


@article{zhang:tsmc12,
    author  = {Haichao Zhang and Yanning Zhang and Nasser M. Nasrabadi and Thomas S. Huang},
    title   = {Joint Structured Sparsity based Classification for Multiple-Measurement Transient Acoustic Signals},
    journal = IEEE_J_SMCB,
    volume  = 42,
    number  = 6,
    year    = 2012,
    pages   = {1586--1598}
}


@inproceedings{yuan:cvpr10,
    author      = {Xiao-Tong Yuan and Shuicheng Yan},
    title       = {Visual classification with multi-task joint sparse representation},
    booktitle   = ieee_cvpr,
    pages       = {3493--3500},
    year        = 2010
}

@misc{adl,
    title   = {{ADL Histopathological Image Data Set}},
    url     = {http://signal.ee.psu.edu/adl.htm}
}



@techreport{srinivas_optprob:techrep12,
  author        = {Umamahesh Srinivas and Yuanming Suo and Minh Dao and Vishal Monga and Trac D. Tran},
  title         = {Spike-and-slab priors for sparse representation-based classification problems},
  institution   = {Pennsylvania State University},
  number        = {PSU-JHU-EE-TR-201201},
  year          = 2012,
  month         = oct,
  url           = {http://signal.ee.psu.edu/techrep/sspic.pdf}
}





@article{yen11b,
  author    =   "Tso-Jung Yen and Yu-Min Yen",
  title     =   "Grouped variable selection via nested spike and slab priors",
  journal   =   {under review}
}


@article{hang:jbb09,
    author = "X. Hang and F.-X. Wu",
    title = "Sparse Representation for Classification of Tumors Using Gene Expression Data",
    journal = "Journal of Biomedicine and Biotechnology",
    volume = 2009,
    year = 2009,
    note = "doi:10.1155/2009/403689"
}




@inproceedings{huang:cvpr08,
    author = "J. Huang and X. Huang and D. Metaxas",
    title = "Simultaneous image transformation and sparse representation recovery",
    booktitle = ieee_cvpr,
    pages = "1--8",
    month = jun,
    year = 2008
}

@article{tropp:tit07,
  author = "J. Tropp and A. Gilbert",
  title =  "Signal recovery from random measurements via Orthogonal Matching Pursuit",
  journal = ieee_tit,
  volume =   53,
  number = 12,
  month =    dec,
  year =     2007,
  pages =    "4655--4666"
}

@article{dai:tit09,
  author = "W. Dai and O. Milenkovic",
  title =  "Subspace Pursuit for Compressive Sensing Signal Reconstruction",
  journal = ieee_tit,
    volume = 55,
    number = 5,
    month = may,
    year = 2009,
    pages = "2230--2249"
}


@article{tan:tsp10,
  author    =   {V.~Y.~F. Tan and S. Sanghavi and J.~W. Fisher III and A.~S. Willsky},
  title     =   {Learning graphical models for hypothesis testing and classification},
  journal   =   {IEEE Trans. Signal Processing},
  year      =   {2010},
  volume    =   {58},
  number    =   {11},
  pages     =   {5481-5495},
  month     = 	{Nov}
}

@book{lauritzen_gm:96,
  title     =   {{Graphical Models}},
  publisher =   {Oxford University Press, NY},
  year      =   {1996},
  author    =   {S.~L. Lauritzen}
}

@article{chow:tit68,
  author    =   {C.~K. Chow and C.~N. Liu},
  title     =   {Approximating discrete probability distributions with dependence trees},
  journal   =   IEEE_J_IT,
  year      =   {1968},
  volume    =   {14},
  number    =   {3},
  pages     =   {462-467}
}

@ARTICLE{wainwright_gm:08,
  title  =       {Graphical Models, Exponential Families and Variational Inference},
  author   =     {M. J. Wainwright and M. I. Jordan},
  journal =      {Foundations and Trends in Machine Learning},
  year    =  2008,
  volume = 1,
  number = "1-2",
  pages = "1-305"
}

@inproceedings{srinivas_facerec:11,
  author    = "U. Srinivas and V. Monga and Y. Chen and T. D. Tran",
  title     = "Sparsity-based face recognition using discriminative graphical models",
  booktitle = "Proc. {IEEE} Asilomar Conf. on Signals, Systems and Computers",
  year      = "2011"
}

@article{baraniuk:pieee10,
  author    =   {R.~G. Baraniuk and V. Cevher and M. Wakin},
  title     =   {Low-dimensional models for dimensionality reduction and signal recovery: {A} geometric perspective},
  journal   =   {{Proc. IEEE}},
  year      =   {2010},
  volume    =   {98},
  number    =   {6},
  pages     =   {959--971}
}




@article{donoho:tit06,
    author = "D. L. Donoho",
    title = "Compressed Sensing",
    journal = ieee_tit,
    volume = 52,
    number = 4,
    year = 2006,
    month = apr,
    pages = "1289--1306"
}





@inproceedings{elhamifar:cvpr09,
    author = "E. Elhamifar and R. Vidal",
    title = "Sparse subspace clustering",
    booktitle = ieee_cvpr,
    pages = "2790--2797",
    month = jun,
    year = 2009
}

@inproceedings{do_2008,
    author = "T. T. Do and L. Gan and N. H. Nguyen and T. D. Tran",
    title = "Sparsity adaptive matching pursuit algorithm for practical compressed sensing",
    booktitle = "Proc. IEEE Asilomar Conf. on Signals, Systems, and Computers",
    month = oct,
    year = 2008,
    pages = "581-587",
    address = "Pacific Grove, CA"
}


@article{
    Pillai_2011,
    author = "J. K. Pillai and V. M. Patel and R. Chellappa and N. Ratha",
    title = "Secure and robust iris recognition using Sparse Representations and Random Projections",
    journal = ieee_tpami,
    volume = 33,
    number = 9,
    month = sep,
    year = 2011,
    pages = "1877--1893"
}


@article{huttenlocher:ijcv05,
    author = "P.~F. Felzenszwalb and D.~P. Huttenlocher",
    title = "Pictorial structures for object recognition",
    journal = {{Int. Journal of Computer Vision}},
    volume = 61,
    number = 1,
    month = Jan,
    year = 2005,
    pages = "55--79"
}

@article{fischler:tc73,
    author = "M.~A. Fischler and R.~A. Elschlager",
    title = "The representation and matching of pictorial structures",
    journal = {{IEEE Trans. Computer}},
    volume = 22,
    number = 1,
    month = Jan,
    year = 1973,
    pages = "67--92"
}


@article{roth:tnn04,
    author = "V. Roth",
    title = "The Generalized {LASSO}",
    journal = ieee_tnn,
    volume = 15,
    year = 2004,
    pages = "16-28"
}

@article{olshausen:nature96,
    author 	= {B.~A. Olshausen and D.~J. Field},
    title 	= {Emergence of Simple-Cell Receptive Field Properties by Learning a Sparse Code for Natural Images},
    journal = {Nature},
    number 	= 381,
    month 	= jul,
    year 	= 1996,
    pages 	= {607--609}
}

@article{zhao:acm03,
    author  = {W. Zhao and R. Chellappa and P.~J. Phillips and A. Rosenfeld},
    title   = {Face recognition: A literature survey},
    journal = {ACM Computing Surveys},
    volume  = 35,
    number  = 4,
    month   = dec,
    year    = 2003,
    pages   = {399--458}
}

@article{georghiades:tpami01,
    author  = {A.~S. Georghiades and P.~N. Belhumeur and D.~J. Kriegman},
    title   = {From few to many: Illumination cone models for face recognition under variable lighting and pose},
    journal = IEEE_J_PAMI,
    month   = jun,
    year    = 2001,
    volume  = 23,
    number  = 6,
    pages   = {643--660}
}

@article{wagner:tpami12,
    author    =   {A. Wagner and J. Wright and A. Ganesh and Z. Zhou and H. Mobahi and Y. Ma},
    title     =   {Towards a practical face recognition system: {R}obust alignment and illumination by sparse representation},
    journal   =   IEEE_J_PAMI,
    month     =   feb,
    year      =   {2012},
    volume    =   {34},
    number    =   {2},
    pages     =   {372--386}
}

@article{turk:jcn91,
    author  = {M. Turk and A. Pentland},
    title   = {Eigenfaces for recognition},
    journal = {J. Cogn. Neurosci.},
    volume  = 3,
    number  = 1,
    year    = 1991,
    pages   = {71--86}
}

@inproceedings{ho:cvpr03,
    author = {J. Ho and M. Yang and J. Lim and K. Lee and D. Kriegman},
    title = {Clustering appearances of objects under varying illumination conditions},
    booktitle = ieee_cvpr,
    month = jun,
    year = {2003},
    pages = {11--18}
}

@book{vapnik:book95,
  author    =   {V.~N. Vapnik},
  title     =   {The nature of statistical learning theory},
  publisher =   {New York, USA: Springer},
  year      =   {1995}
}

@article{belhumeur:tpami97,
    author  = {P.~N. Belhumeur and J.~P. Hespanha and D.~J. Kriegman},
    title   = {Eigenfaces vs. Fisherfaces: Recognition using class specific linear projection},
    journal = IEEE_J_PAMI,
    volume  = 19,
    number  = 7,
    month   = jul,
    year    = 1997,
    pages   = {711--720}
}

@article{martinez:techrep98,
    author  = {A.~M. Martinez and R. Benavente},
    title   = {{The AR face database}},
    journal = {CVC Tech. Report},
    year    = 1998,
    number  = 24
}


@inproceedings{fei:cvpr04,
    author      = {L. Fei-Fei and R. Fergus and P. Perona},
    title       = {{Learning generative visual models from few training examples: An incremental Bayesian approach tested on 101 object categories}},
    booktitle   = ieee_cvpr,
    year        = {2004},
    pages       = {59--70}
}

@inproceedings{zhang:cvpr06,
    author      = {H. Zhang and A. Berg and M. Maire and J. Malik},
    title       = {{SVM-KNN: Discriminative nearest neighbor classification for visual category recognition}},
    booktitle   = ieee_cvpr,
    year        = {2006},
    pages       = {2126--2136}
}

@inproceedings{lazebnik:cvpr06,
    author      = {S. Lazebnik and C. Schmid and J. Ponce},
    title       = {Beyond bags of features: {S}patial pyramid matching for recognizing natural scene categories},
    booktitle   = ieee_cvpr,
    year        = {2006},
    pages       = {2169--2178}
}

@inproceedings{wang:cvpr10,
    author      = {Jinjun Wang and Jianchao Yang and Kai Yu and Fengjun Lv and Thomas Huang and Yihong Gong},
    title       = {Locality-constrained linear coding for image classification},
    booktitle   = ieee_cvpr,
    year        = {2010}
}

@inproceedings{nilsback:cvpr06,
    author      = {M. Nilsback and A. Zisserman},
    title       = {A visual vocabulary for flower classification},
    booktitle   = ieee_cvpr,
    year        = {2006},
    pages       = {1447--1454}
}



@article{yuan:tip12,
    author  = {Xiao-Tong Yuan and Xiaobai Liu and Shuicheng Yan},
    title   = {Visual classification with multitask joint sparse representation},
    journal = IEEE_J_IP,
    volume  = 21,
    number  = 10,
    year    = 2012,
    pages   = {4349--4360}
}


@inproceedings{chen:cvpr12,
    author      = {Qiang Chen and Zheng Song and Yang Hua and Zhongyang Huang and Shuicheng Yan},
    title       = {Hierarchical matching with side information for image classification},
    booktitle   = ieee_cvpr,
    year        = {2012},
    pages       = {3426--3433}
}

@inproceedings{chai:iccv11,
    author      = {Yuning Chai and Victor Lempitsky and Andrew Zisserman},
    title       = {{BiCoS: A Bi-level Co-Segmentation Method for Image Classification}},
    booktitle   = {Proc. IEEE Conf. Comput. Vision},
    year        = {2011},
    pages       = {2579--2586}
}


@inproceedings{kanan:cvpr10,
    author      = {C. Kanan and G. Cottrell},
    title       = {Robust classification of objects, faces, and ﬂowers using natural image statistics},
    booktitle   = ieee_cvpr,
    year        = {2010},
    pages       = {2472--2479}
}

@inproceedings{gehler:iccv09,
    author      = {P. Gehler and S. Nowozin},
    title       = {On feature combination for multiclass object classification},
    booktitle   = {Proc. IEEE Conf. Comput. Vision},
    year        = {2009},
    pages       = {221--228}
}


@inproceedings{srinivas:icip13,
  author    = {U. Srinivas and Y. Suo and M. Dao and V. Monga and T.~D. Tran},
  title     = {Structured sparse priors for image classification},
  booktitle = ieee_icip,
  year      = {2013}
}

@inproceedings{yu:isbi11,
    author      =   {Yang Yu and Junzhou Huang and Shaoting Zhang and Christophe Restif and Xiaolei Huang and Dimitris Metaxas},
    title       =   {Group sparsity based classification for cervigram segmentation},
    booktitle   =   {Proc. IEEE Int. Symp. Biomed. Imag.},
    year        =   2011,
    pages       =   {1425--1429}
}


@article{yuan:jrss07,
    author  = {M. Yuan and Y. Lin},
    title   = {Model selection and estimation in regression with grouped variables},
    journal = {J. Royal Stat. Soc. B},
    volume  = 68,
    number  = 1,
    year    = 2007,
    pages   = {49--67}
}


@inproceedings{majumdar:icassp09,
  author    = {A. Majumdar and R.~K. Ward},
  title     = {Classification via group sparsity promoting regularization},
  booktitle = ieee_icassp,
  year      = {2009},
  pages     = {861--864}
}


@article{sprechmann:tsp11,
    author  =   {P. Sprechmann and I. Ramirez and G. Sapiro and Y.~C. Eldar},
    title   =   {C-{H}i{L}asso: {A} collaborative hierarchical sparse modeling framework},
    journal =   IEEE_J_SP,
    volume  =   59,
    number  =   9,
    month   =   sep,
    year    =   2011,
    pages   =   {4183--4198}
}

@article{tropp:sp06a,
    author  =   {J.~A. Tropp and A.~C. Gilbert and M.~J. Strauss},
    title   =   {Algorithms for simultaneous sparse approximation. {Part I}: Greedy pursuit},
    journal =   {Signal Processing},
    month   =   apr,
    year    =   2006,
    volume  =   86,
    pages   =   {572--588}
}

@inproceedings{yang:icip10,
    author      =   {Allen Y. Yang and A. Ganesh and S. Shankar Sastry and Yi Ma},
    title       =   {Fast $l_1$-minimization algorithms and an application in robust face recognition: {A} review},
    booktitle   =   {Proc. IEEE Int. Conf. Image Processing},
    year        =   2010,
    pages       =   {1849--1852}
}

@inproceedings{suo:icassp13,
  author    = {Y. Suo and M. Dao and T.~D. Tran and U. Srinivas and V. Monga},
  title     = {Hierarchical sparse modeling using spike and slab priors},
  booktitle = ieee_icassp,
  year      = {2013},
  pages     = {3103--3107}
}

@article{majumdar:prl10,
    author  =   {A. Majumdar and R.~K. Ward},
    title   =   {Improved group sparse classifier},
    journal =   {Pattern Recogn. Lett.},
    month   =   oct,
    year    =   2010,
    volume  =   31,
		number	=		13,
    pages   =   {1959--1964}
}

@inproceedings{chouzenoux:icip11,
  author    = {E. Chouzenoux and J.-C. Pesquet and H. Talbot and A. Jezierska},
  title     = {A memory gradient algorithm for $l_2-l_0$ regularization with applications to image restoration},
  booktitle = ieee_icip,
  year      = {2011},
  pages     = {2717--2720}
}

@article{chouzenoux:siam13,
    author  =   {E. Chouzenoux and A. Jezierska and J. Pesquet and H. Talbot},
    title   =   {A majorize-minimize subspace approach for $l_2-l_0$ image regularization},
    journal =   {SIAM J. Imaging Sci.},
    year    =   2013,
    volume  =   6,
	number	=	1,
    pages   =   {563--591}
}


==> SupplementaryMaterial/Dedication.tex <==
To my beloved parents

==> SupplementaryMaterial/ListOfSymbols.tex <==
% Place the list of symbols below.
\begin{eqlist}[\def\makelabel#1{\hfill#1}\labelsep 1em]

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, but we should really add some more text, though we need it to go on two lines, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\end{eqlist}

==> eqparbox/README <==
                  +--------------------------------+
                  |EQPARBOX: Equal-widthed parboxes|
                  |By Scott Pakin <pakin@uiuc.edu> |
                  +--------------------------------+


Description
-----------

LaTeX users sometimes need to ensure that two or more blocks of text
occupy the same amount of horizontal space on the page.  To that end,
the eqparbox package defines a new command, \eqparbox, which works
just like \parbox, except that instead of specifying a width, one
specifies a tag.  All eqparboxes with the same tag -- regardless of
where they are in the document -- will stretch to fit the widest
eqparbox with that tag.  This simple, equal-width mechanism can be
used for a variety of alignment purposes, as is evidenced by the
examples in eqparbox's documentation.


Installation
------------

There's nothing special about building eqparbox:

    latex eqparbox.ins     <== Generate eqparbox.sty
    latex eqparbox.dtx     <== Produce the documentation (eqparbox.dvi)
    latex eqparbox.dtx     <== Again, to get labels and eqparboxes right
    makeindex -s gind.ist eqparbox    <== Generate an index
    latex eqparbox.dtx     <== Incorporate the index into the document

If you're new to this, see
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=instpackages for more
information on installing packages.


Copyright and license
---------------------
Copyright (C) 2001 Scott Pakin <pakin@uiuc.edu>

This package may be distributed and/or modified under the conditions
of the LaTeX Project Public License, either version 1.2 of this
license or (at your option) any later version.  The latest version of
this license is in:

    http://www.latex-project.org/lppl.txt

and version 1.2 or later is part of all distributions of LaTeX version
1999/12/01 or later.

